Scalable Optimal Transport Methods in Machine Learning: A Contemporary Survey

Optimal Transport (OT) is a mathematical framework that first emerged in the eighteenth century and has led to a plethora of methods for answering many theoretical and applied questions. The last decade has been a witness to the remarkable contributions of this classical optimization problem to machine learning. This paper is about where and how optimal transport is used in machine learning with a focus on the question of scalable optimal transport. We provide a comprehensive survey of optimal transport while ensuring an accessible presentation as permitted by the nature of the topic and the context. First, we explain the optimal transport background and introduce different flavors (i.e., mathematical formulations), properties, and notable applications. We then address the fundamental question of how to scale optimal transport to cope with the current demands of big and high dimensional data. We conduct a systematic analysis of the methods used in the literature for scaling OT and present the findings in a unified taxonomy. We conclude with presenting some open challenges and discussing potential future research directions. A live repository of related OT research papers is maintained in https://github.com/abdelwahed/OT_for_big_data.git

==> sections/7-app_kr_norm.tex <==

%% appendaix A

\section{Kantorovich-Rubinstein Proof} \label{sec:app_kr_norm}

Let's recall the \textit{semi-dual} \eqref{eq:sd} and the \textit{Kantorovich-Rubinstein} \eqref{eq:kr} formulations:

\begin{align*}
    &\sup\limits_{\varphi \in L^1(\mu), \varphi \in L^1(\nu)} &\Big[ \int_{\mathbb{X}} \varphi(x) d\mu(x)  + \int_{\mathbb{Y}} \varphi^{c}(y) d \nu(y) \Big] \label{eq:sd} \tag{\text{SD}} \\
   &\sup\limits_{\varphi \in L_d(1)} &\Big[ \int_{\mathbb{X}} \varphi(x) d\mu(x) - \int_{\mathbb{Y}} \varphi(y) d \nu(y) \Big] \label{eq:kr} \tag{\text{KR}} 
\end{align*}

\textbf{Proof}. To prove the equivalence of the above formulations when $m = d$ is a distance function satisfying the triangle inequality, we need to prove the following:
\begin{enumerate}
    \item If $\varphi$ is 1-Lipschitz, then $\varphi$ is integrable.
    \item If $\varphi$ is integrable and optimal in the semi-dual formulation, then $\varphi$ is 1-Lipschitz.
    \item The optimal solution $\varphi$ satisfies $\varphi^c = -\varphi$.
\end{enumerate}
The first statement says that the 1-Lipschitz constraint implies semi-dual feasibility. The second statement says that the optimal solution to the semi-dual must be 1-Lipschitz. Given these 2 statements, one can restrict the search to the space of 1-Lipschitz functions without risk of cutting out the optimal solution $\varphi$ or violating the original semi-dual constraint. Finally, the third statement says that we can replace the c-transform of the function by its negation.

Proving the first statement is simple because 1-Lipschitz functions must be continuous by definition which implies that the function is integrable.

To prove the second statement, we start by proving $(\varphi^{c})^{c} = \varphi$ for the optimal $\varphi$ which is an important intermediate result. Given the original dual formulation, if we fix any feasible function $\varphi(X)$, the optimal $\psi(Y)$ is $\psi(Y) = \inf\limits_{X} [ d(X,Y) - \varphi(X)] = \varphi^c(Y)$ because this is the maximum value $\psi$ can take for each $Y$ without violating the constraint $\varphi(X) + \psi(Y) \leq d(X, Y)$. Similarly, one can fix $\psi(Y)$ and derive the optimal $\varphi(X) = \inf\limits_{Y} [ d(X,Y) - \psi(Y)] = \psi^c(X)$. So the optimal $\varphi(X)$ and $\psi(Y)$ satisfy the following relationships:
\begin{align*}
    \psi(Y) & = \varphi^c(Y) \\
    \varphi(X) & = \psi^c(X)
\end{align*}
Given that each \textit{optimal} function is the c-transform of another function, the optimal $\psi$ and $\varphi$ are so-called c-convex functions by definition \cite{Berlin2009OptimalNew}. Using proposition 5.8 in \cite{Berlin2009OptimalNew}, a function $f$ is c-convex if and only if $(f^{c})^{c} = f$.

We then prove that $\varphi^c$ is 1-Lipschitz. 
\begin{multline*}
    |\varphi^{c}(X) - \varphi^{c}(Y)| = \\
        \Big| \inf\limits_{Z} [ d(X,Z) - \varphi(Z)] - \inf\limits_{Z} [ d(Y,Z) - \varphi(Z)] \Big|
\end{multline*}
Given the general inequality:
\begin{align*}
    |\inf\limits_{x} f(x) - \inf\limits_{x} g(x)| \leq \sup\limits_{x} |f(x) - g(x)|
\end{align*}
it follows that:
\begin{align*}
    |\varphi^{c}(X) - \varphi^{c}(Y)| & \leq \sup\limits_{Z} |d(X, Z) - d(Y, Z)|
\end{align*}
Using the triangle inequality for $d$:
\begin{align*}
    d(X, Z) & \leq d(X, Y) + d(Y, Z) \\
    d(X, Z) - d(Y, Z) & \leq d(X, Y)
\end{align*}
it follows that:
\begin{align*}
    |\varphi^{c}(X) - \varphi^{c}(Y)| & \leq \sup\limits_{Z} |d(X, Z) - d(Y, Z)| \\
    & \leq \sup\limits_{Z} |d(X, Y)| \\
    & = d(X, Y)
\end{align*}
This completes the proof that $\varphi^{c}$ is 1-Lipschitz w.r.t. $d$. One can then replicate the above derivations for $(\varphi^{c})^{c}$ proving it is 1-Lipschitz. Therefore, $\varphi$ is 1-Lipschitz.

To conclude, we prove that when $m = d$ is a distance function, $\varphi^c = -\varphi$. To prove this, we can prove the following:
\begin{enumerate}
    \item $\varphi^c \leq -\varphi$
    \item $\varphi^c \geq -\varphi$
\end{enumerate}
To prove the first, let's start with the definition of $\varphi^c$:
\begin{align*}
    \varphi^c(Y) & = \inf\limits_{X} [ d(X,Y) - \varphi(X)] \\
    & \leq d(X^0,Y) - \varphi(X^0)
\end{align*}
for any particular choice $X^0$. Setting $X^0 = Y$, we get $\varphi^c(Y) \leq - \varphi(Y)$.

To prove the second inequality, we invoke the previous result that the optimal $\varphi$ is 1-Lipschitz.
\begin{align*}
    |\varphi(X) - \varphi(Y)| & \leq d(X, Y) \\
    \varphi(X) - \varphi(Y) & \leq d(X, Y) \\
    -\varphi(X) & \geq -d(X, Y) - \varphi(Y)
\end{align*}
Using this result and the definition of $\varphi^c(Y)$, we get:
\begin{align*}
    \varphi^c(Y) & = \inf\limits_{X} [ d(X,Y) - \varphi(X)] \\
    & \geq \inf\limits_{X} [ d(X,Y) - d(X, Y) - \varphi(Y)] \\
    & = \inf\limits_{X} - \varphi(Y) \\
    & = - \varphi(Y)
\end{align*}
This completes the proof.

\textbf{Same Function, Different Values}. Note that while the functional form of $\varphi$ is the same for both terms in the dual formulation's objective (when $m = d$), in the discrete case (when the supports $\mathbb{X}$ and $\mathbb{Y}$ are different), two different sets of dual values corresponding to $\mathbb{X}$ and $\mathbb{Y}$ are still needed. So the semi-dual formulation is mostly useful when we have finite, discrete and common supports in the 2 measures, e.g. $\mathbb{X} = \mathbb{Y} = \{0, 1\}$, or if a continuous parameterization for the functional form of $\varphi$ is used instead of a tabular parameterization which maps each $X \in \mathbb{X}$ (or $Y \in \mathbb{Y}$) to a potentially unique value $\varphi(X)$ (or $\varphi(Y)$).

\textbf{Notation Discrepancy} In some other works including Cedric Villani's book\cite{Berlin2009OptimalNew}, their $\varphi$ is our $\psi$ and their $\psi$ is our $-\varphi$. So a few things look different:
\begin{itemize}
    \item The original dual objective function becomes:
    \begin{align*}
        \mathbb{E}_{Y \sim \nu} \big[ \varphi(Y) \big] - \mathbb{E}_{X \sim \mu} \big[ \psi(X) \big]
    \end{align*}
    \item The dual constraint becomes:
    \begin{align*}
        \varphi(Y) - \psi(X) \leq m(X, Y)
    \end{align*}
    \item The c-transform becomes:
    \begin{align*}
        \varphi(Y) = \psi^{c}(Y) = \inf\limits_{X} [ m(X,Y) + \psi(X)]
    \end{align*}
    \item The semi-dual objective function becomes:
    \begin{align*}
        \mathbb{E}_{Y \sim \nu} \big[ \psi^{c}(Y) \big] - \mathbb{E}_{X \sim \mu} \big[ \psi(X) \big]
    \end{align*}
    \item In the special case when $m(x, y) = d(x, y)$ is a distance function, the c-transform becomes:
    \begin{align*}
        \varphi(Y) = \psi^{c}(Y) = \psi(Y)
    \end{align*}
    \item In the same special case, the semi-dual objective function in terms of $\psi \in L_d(1)$ becomes:
    \begin{align*}
        \mathbb{E}_{Y \sim \nu} \big[ \psi(Y) \big] - \mathbb{E}_{X \sim \mu} \big[ \psi(X) \big]
    \end{align*}
\end{itemize}


==> sections/pc_matching.tex <==

\subsubsection{Point Cloud Matching}
\label{sec:pc_matching}

One is often interested in computing with a collection of point clouds given correspondences between the point clouds. An example of computing with a sparse point cloud is the problem of bundle adjustment~\cite{triggs1999bundle}. Here one jointly determines the 3D world coordinates of a set of landmarks and the pose and intrinsic parameters of a collection of cameras given a set of 2D pixel image coordinates of those landmarks for each camera. A simplifying assumption is that correspondences between the 2D image coordinates of landmarks between different cameras is known. The association problem is hard because it is discrete and combinatorial in nature; for $n$ landmarks and $m$ cameras there are $n^m$ possible associations. This means that, without relaxing the problem, gradient-based methods cannot solve the problem and naive exhaustive search is intractable. Furthermore, when such problems are solved as part of a larger pipeline as is often the case in bundle adjustment, these computational difficulties are compounded. Classical relaxations to this problem lead to algorithms such as the iterative closest point algorithm, which \cite{LeeHierarchicalAlignment} can be sensitive to initial conditions.

A promising way to relax the point cloud association problem is through optimal transport. This approach offers several advantages: the problem can be solved using gradient-based optimisers, the problem is no longer combinatorial, and the problem can be included in a larger pipeline and solved jointly with a downstream task through implicit differentiation (see~\cref{sec:scaling_stochastic}).

The blind perspective-n-point (PnP) problem is to determine the pose of a camera given a point cloud of 2D pixel image coordinates from the camera and a 3D point cloud of the environment without any correspondences between the two point clouds. Blind PnP is approached in~\cite{liu2020learning} by extracting $d=128$ dimensional neural network features for the 2D and 3D point clouds and then using the sinkhorn algorithm to estimate an optimal transport plan. Here the ground cost is the Euclidean distance between neural network features. The top $K$ elements of the optimal transport plan are taken to be correspondences, which can then be passed to a standard camera pose estimation framework. Very similar approaches to the association problem are also taken by~\cite{sarlin2020superglue,simon2020stickypillars,yew2020rpm}, without focusing on the blind PnP problem and 2D-3D correspondences. While iterates of the Sink-horn algorithm are differentiable, leading to an end-to-end differentiable pipeline, gradients of the optimal transport plan can be computed without differentiating through the sinkhorn algorithm~\cite{capmbell2020pnp}.
% , see \S~\ref{sec:implicit}.

\iffalse
Experimental results \cite{LeeHierarchicalAlignment} demonstrates that Iterative Closest Point(ICP)\cite{} is notorious for being dependent on good initial conditions.


Recently, researchers~\cite{liu2020learning,sarlin2020superglue, simon2020stickypillars} bring the Sinkhorn's algorithm \cite{cuturi2013sinkhorn} to this matching task for its end-to-end training ability.
RPM-Net \cite{yew2020rpm} uses Sinkhorn \cite{sinkhorn1964relationship} to obtain soft correspondences between source and target frame to increase robustness to non-overlapping points. One-shot \cite{dang2020learning} pads outlier bins to Sinkhorn to further improve robustness.
\fi

